LGBT+ Inclusivity in Physics and Astronomy: A Best Practices Guide

We present the second edition of a Best Practices Guide for academic departments and other institutions striving to create more inclusive environments for physicists and astronomers in the LGBT+ community. Our recommendations incorporate new research since the original, 2014 edition, and are designed for anyone who wishes to become aware of -- and help mitigate -- the extra burdens that face members of the LGBT+ community in the physical sciences.

==> fair_benefits.tex <==
\subsection {Provide other benefits fairly}
\label{other-benefits}
 \BPGtag{U}
% tags: U, I
% vvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvvv
Offer other benefits equally to both different-gender and same-gender spouses/partners of employees.  These benefits may include access to the gym, the library, and the university credit union.  If child care is provided on campus, make it easy for both parents to take their child home.  If your country or region recognizes same-gender marriage, implement policies to support same-gender couples who have recently arrived from less-friendly countries.  Ensure that parental leave policies provide support for a student, staff member, or faculty member who has recently welcomed a child to their family, whether or not that individual is a cisgender woman who physically gave birth.
% ^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^^


==> tags.tex <==
\section {BPG Tags}
\label{taglist}

This page is a list of all tags. To tag something, use the command
\begin{verbatim}
\BPGtag{tagname},
\end{verbatim}
where tagname is a single letter, chosen from the following:
\begin{itemize}
\item $[D]$epartment level: Advice for fostering a welcoming and supportive department including 
guidelines for department chairs,
administrators, individual members, and staff. \BPGtag{D}

\item $[C]$lassroom: Advice for improving the climate in classrooms and other sites of instruction. 
\BPGtag{C}

\item $[A]$dvisors and Mentors:  Advising and mentoring relationships between faculty, 
postdoctoral research associates, graduate and undergraduate students, and staff. \BPGtag{A}

\item $[H]$iring and promotions: Suggestions for best practices during hiring and promotions. 
\BPGtag{H}

\item $[T]$ravel:  Advice regarding travel, including to regions with different laws and customs. 
\BPGtag{T}

\item $[I]$nstitution level: Advice for promoting healthy institutional practices, including 
guidelines for administrators and deans. \BPGtag{I}
 
\item $[R]$esearch groups and collaborations: Advice for sustaining healthy research groups and 
collaborations, including guidelines for group leaders and principal investigators.  \BPGtag{R}
 
\item $[S]$taff: Advice for Staff for establishing a welcoming work environment within their 
institution. \BPGtag{S}

%\item $[W]$orkshops \& conferences: Advice for organizing or hosting conferences by a unit and/or 
%an institution. \BPGtag{W}

\item $[P]$ompliance: Internal tag for compliance with recommended or quantifiable best practices 
-- items that will go on Best Practices guide checklists. Only visible to editors. \BPGtag{P}

\end{itemize}
